The Blessings of Multiple Causes

Causal inference from observational data often assumes "ignorability," that all confounders are observed. This assumption is standard yet untestable. However, many scientific studies involve multiple causes, different variables whose effects are simultaneously of interest. We propose the deconfounder, an algorithm that combines unsupervised machine learning and predictive model checking to perform causal inference in multiple-cause settings. The deconfounder infers a latent variable as a substitute for unobserved confounders and then uses that substitute to perform causal inference. We develop theory for the deconfounder, and show that it requires weaker assumptions than classical causal inference. We analyze its performance in three types of studies: semi-simulated data around smoking and lung cancer, semi-simulated data around genome-wide association studies, and a real dataset about actors and movie revenue. The deconfounder provides a checkable approach to estimating closer-to-truth causal effects.

==> table1_jamesbond.tex <==

\begin{table*}[ht]
\scriptsize
  \begin{center}
    \begin{tabular}{lp{10mm}p{9mm}p{10mm}p{12mm}p{9mm}p{9mm}p{9mm}p{9mm}p{11mm}r} 
     \toprule
Movie& Sean Connery & Roger Moore & Pierce Brosnan &  Desmond Llewelyn & Lois Maxwell & Bernard Lee & William Forsythe& Horatio Sanz & Carey Mulligan & Revenue\\
          \midrule
Goldfinger & 1 & 0 & 0 & 1 & 1& 1&0 & 0 & 0 & 124m\\
A View to a Kill & 0 & 1 & 0 &1 & 1& 0 & 0 & 0 & 0 & 152m\\
The Rock & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 660m\\
Diamonds are Forever & 1 & 0 & 0 & 1 & 1& 1&0 & 0 & 0 & 116m\\
Boat Trip & 0 & 1 & 0 & 0 & 0 & 0  & 0 & 1 & 0 & 8m \\
Tomorrow Never Dies & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 333m\\
Never Say Never Again & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 160m\\
The Greatest & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 &1 &1m\\
Live and Let Die & 0 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 161m\\
Dr. No & 1 & 0 & 0 & 0 & 1 & 1& 0 & 0 & 0 & 59m\\
Money Never Sleeps & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 134m \\
For Your Eyes Only & 0 &1 & 0 & 1 & 1& 0 & 0 & 0 & 0 &195m\\
      \bottomrule
    \end{tabular}
    \caption{How casts cause movie earnings?: Actors as the (multiple) causes and
    revenue as the outcome. \label{tab:tab1_jamebond}}
  \end{center}
\end{table*}

==> table4_bottomrevmov.tex <==
% !TEX root = latent_confounder.tex

\begin{table*}[ht]
\scriptsize
  \begin{center}
    \begin{tabular}{llr} 
     \toprule
        Title & Cast & Revenue\\
        \midrule
        \emph{My Baby's Daddy}&\{Eddie Griffin, Anthony Anderson, Michael Imperioli, Method Man, $\ldots$ \}&\$51\\
        \emph{When Did You Last See Your Father?}&\{Jim Broadbent, Colin Firth, Juliet Stevenson, Gina McKee, $\ldots$ \}&\$92\\
        \emph{Rugrats in Paris: The Movie}&\{E.G. Daily, Susan Sarandon, John Lithgow, Tara Strong, $\ldots$ \}&\$103\\
        \emph{Khiladi 786}&\{Akshay Kumar, Asin Thottumkal, Himesh Reshammiya, Mithun Chakraborty, $\ldots$ \}&\$126\\
        \emph{I Married a Strange Person!}&\{Charis Michelsen, Tom Larson, Richard Spore\}&\$203\\
        \emph{Irreversible}&\{Monica Bellucci, Vincent Cassel, Albert Dupontel, Jo Prestia, $\ldots$ \}&\$792\\
        \emph{Eddie: The Sleepwalking Cannibal}&\{Thure Lindhardt, Dylan Smith, Georgina Reilly, Alain Goulem, $\ldots$ \}&\$1632\\
        \emph{Mi America}&\{Robert Fontaine, Michael Brainard, Grant Boyd, Michael Derek, $\ldots$ \}&\$3330\\
        \emph{The Adventurer: The Curse of the Midas Box}&\{Aneurin Barnard, Michael Sheen, Lena Headey, Sam Neill, $\ldots$ \}&\$6399\\
        \emph{Special}&\{Michael Rapaport, Josh Peck, Robert Baker, Jack Kehler, $\ldots$ \}&\$7202\\
        \emph{Janky Promoters}&\{Ice Cube, Mike Epps, Young Jeezy, Darris Love, $\ldots$ \}&\$9069\\
        \emph{Down Terrace}&\{Robert Hill, Robin Hill, Julia Deakin, David Schaal, $\ldots$ \}&\$10000\\
        \emph{Alone With Her}&\{Colin Hanks, Ana Claudia Talancfn, Jordana Spiro, Jonathon Trent, $\ldots$ \}&\$10018\\
        \emph{Naturally Native}&\{Valerie Red-Horse, Yvonne Russo", Irene Bedard, Kimberly Guerrero, $\ldots$ \}&\$10508\\
        \emph{The Perfect Host}&\{David Hyde Pierce, Clayne Crawford, Nathaniel Parker, Helen Reddy\}&\$14870\\
        \emph{Major Dundee}&\{Charlton Heston, Richard Harris, Jim Hutton, James Coburn, $\ldots$ \}&\$14873\\
        \emph{Strangerland}&\{Nicole Kidman, Joseph Fiennes, Hugo Weaving, Lisa Flanagan, $\ldots$ \}&\$17472\\
        \emph{5 Days of War}&\{Rupert Friend, Val Kilmer, Andy Garceda, Dean Cain, $\ldots$ \}&\$17479\\
        \emph{The Good Night}&\{Penelope Cruz, Martin Freeman, Gwyneth Paltrow, Simon Pegg, $\ldots$ \}&\$20380\\
        \emph{The Divide}&\{Lauren German, Michael Biehn, Milo Ventimiglia, Courtney B. Vance, $\ldots$ \}&\$22000\\
        \bottomrule
    \end{tabular}
    \caption{Bottom revenue movies \label{tab:bottomrevmov}}
  \end{center}
\end{table*}
